The potential of CMS as a high-energy neutrino scattering experiment

With its enormous number of produced neutrinos the LHC is a prime facility to study the behaviour of high-energy neutrinos. In this paper we propose a novel search strategy for identifying neutrino scattering via displaced appearing jets in the high granularity calorimeter (HGCAL) of the CMS endcap in the high luminosity run of the LHC. We demonstrate in a cut-and-count based analysis how the enormous hadronic background can be reduced while keeping most of the neutrino signal. This paper serves as a proof-of-principle study to illustrate the feasibility of the first direct observation of high-energetic neutrinos coming from $W$ decays.

==> header.tex <==
\RequirePackage[colorlinks=true
,urlcolor=blue
,anchorcolor=blue
,citecolor=blue
,filecolor=blue
,linkcolor=blue
,menucolor=blue
,linktocpage=true
,pdfproducer=medialab
,pdfa=true
]{hyperref}

\usepackage{amsmath,amssymb,amsthm,amsfonts}
\usepackage{graphicx,tabularx}
\usepackage{color}
\usepackage{multirow}
\usepackage{comment}
\usepackage{enumitem}
\usepackage{cleveref}
\usepackage{slashed}
\usepackage[normalem]{ulem}
\usepackage{scalerel}

\setlist[description]{leftmargin=0.3cm}
\setlist[itemize]{leftmargin=0.5cm}

\newcommand{\be}{\begin{equation} \begin{aligned}}
\newcommand{\ee}{\end{aligned} \end{equation}}
\newcommand{\beqa}{\begin{eqnarray}}
\newcommand{\eeqa}{\end{eqnarray}}

\def\figureautorefname~#1\null{Fig.\,#1\null}
\def\tableautorefname~#1\null{Tab.\,#1\null}
\renewcommand{\sectionautorefname}{Sec.}
\renewcommand{\subsectionautorefname}{Sec.}
\def\equationautorefname~#1\null{Eq.\,(#1)\null}

% General symbols
\newcommand{\im}{\mathrm{i}}
\newcommand{\diff}{\mathrm{d}}
\newcommand{\eg}{{e.\,g.}~}
\newcommand{\ie}{{i.\,e.}~}
\newcommand{\equivalent}{\simeq}
\newcommand{\br}{\mathrm{BR}}

% Units
\newcommand{\ev}{\text{eV}}
\newcommand{\kev}{\text{keV}}
\newcommand{\mev}{\text{MeV}}
\newcommand{\gev}{\text{GeV}}
\newcommand{\tev}{\text{TeV}}

\newcommand{\ab}{\text{ab}}
\newcommand{\iab}{\text{ab}^{-1}}
\newcommand{\fb}{\text{fb}}
\newcommand{\ifb}{\text{fb}^{-1}}
\newcommand{\pb}{\text{pb}}
\newcommand{\ipb}{\text{pb}^{-1}}

\newcommand{\nm}{\text{nm}}
\newcommand{\micm}{\mu\text{m}}
\newcommand{\mm}{\text{mm}}
\newcommand{\cm}{\text{cm}}
\newcommand{\m}{\text{m}}
\newcommand{\km}{\text{km}}

\newcommand{\mrad}{\text{mrad}}
\newcommand{\murad}{\mu\text{rad}}

\newcommand{\g}{\text{g}}
\newcommand{\kg}{\text{kg}}
\newcommand{\ton}{\text{t}}
\newcommand{\sr}{\text{sr}}
\newcommand{\ns}{\text{ns}}

\newcommand{\fasernu}{FASER$\nu$~}

\newcommand{\Eqref}[1]{Equation~(\ref{eq:#1})}
\newcommand{\Eqsref}[2]{Equations~(\ref{eq:#1}) and (\ref{eq:#2})}
\renewcommand{\eqref}[1]{Eq.~(\ref{eq:#1})}
\newcommand{\eqsref}[2]{Eqs.~(\ref{eq:#1}) and (\ref{eq:#2})}
\newcommand{\secref}[1]{Sec.~\ref{sec:#1}}
\newcommand{\secsref}[2]{Secs.~\ref{sec:#1} and \ref{sec:#2}}
\newcommand{\Secref}[1]{Section~\ref{sec:#1}}
\newcommand{\Secsref}[2]{Sections~\ref{sec:#1} and \ref{sec:#2}}
\newcommand{\figref}[1]{Fig.~\ref{fig:#1}}
\newcommand{\figsref}[2]{Figs.~\ref{fig:#1} and \ref{fig:#2}}
\newcommand{\figssref}[3]{Figs.~\ref{fig:#1}, \ref{fig:#2} and \ref{fig:#3}}
\newcommand{\Figref}[1]{Figure~\ref{fig:#1}}
\newcommand{\tableref}[1]{Table~\ref{table:#1}}
\newcommand{\tablesref}[2]{Tables~\ref{table:#1} and \ref{table:#2}}
\newcommand{\appref}[1]{Appendix~\ref{sec:#1}}
\newcommand{\appsref}[2]{Appendices~\ref{sec:#1} and \ref{sec:#2}}


%comments
\RequirePackage[normalem]{ulem} 
\newcommand{\changed}[2]{{\protect\color{red}\sout{#1}}{\protect\color{blue}\uwave{#2}}}

% Define commenting commands
\newcommand{\Felix}[1]{\textcolor{magenta}{FK:#1}}
\newcommand{\PR}[1]{\textcolor{green}{{[ PR: #1]}}}
\newcommand{\PF}[1]{\textcolor{blue}{{[ PF: #1]}}}

\crefname{section}{Sec.}{Secs.}
\crefname{figure}{Fig.}{Figs.}
\crefname{equation}{Eq.}{Eqs.}
\crefname{appendix}{Appendix}{Appendices}
\crefname{table}{Table}{Tables}

%Ref Style
\bibliographystyle{utphys}


==> incl_declare.tex <==


% \tikzstyle{generator} = [rectangle, rounded corners, minimum width=3cm, minimum height=1cm,text centered, draw=Gcolor]
% \tikzstyle{discriminator} = [rectangle, rounded corners, minimum width=3cm, minimum height=1cm,text centered, draw=Dcolor]
% \tikzstyle{io} = [circle, trapezium left angle=70, trapezium right angle=110, minimum width=1cm, minimum height=1cm, text centered, draw=black]

% \tikzstyle{process} = [rectangle, minimum width=1cm, minimum height=1cm, text centered, draw=black]
% \tikzstyle{decision} = [rectangle, minimum width=1cm, minimum height=1cm, text centered, draw=black]

% \tikzstyle{arrow} = [thick,->,>=stealth]

% \usepackage{xcolor}

%% macros for marking changes
\marginparwidth 3.0cm
%\setlength{\hoffset}{-1.6cm}
\newcommand{\mpar}[1]{\rule{2pt}{10pt}
                      {\marginpar{\hbadness10000\flushleft
                      \sloppy\hfuzz10pt\boldmath\footnotesize#1}}
                       \typeout{marginpar: #1}\ignorespaces}
%\def\mda{\mpar{\hfil$\downarrow$\hfil}\ignorespaces}
%\def\mua{\mpar{\hfil$\uparrow$\hfil}\ignorespaces}
%\def\mla{\marginpar[\boldmath\hfil$\rightarrow$\hfil]
%                   {\boldmath\hfil$\leftarrow $\hfil}
%                    \typeout{marginpar: $\leftrightarrow$}\ignorespaces}

% hyper-link hep-ph references
\newcommand{\arxiv}[1]{\href{http://arxiv.org/abs/#1}{arXiv:#1}}
\newcommand{\urlx}[1]{\href{#1}{#1}}
\newcommand{\doix}[2]{\href{http://dx.doi.org/#2}{#1}}

\setlength{\tabcolsep}{2pt}

%\newcommand*{\thead}[1]{\multicolumn{1}{c}{\bfseries #1}}

\def\contentsname{{\normalsize Content}}
\def\tablename{Table}
\def\figurename{Figure}

\def\cls{\text{CL}_\text{s}}
\def\mtr{\overline{m}_t}
\def\pveto{P_\text{veto}}
\def\nj{N_\text{jets}}
\def\meff{m_\text{eff}}
\def\ptmin{p_T^\text{min}}
\def\gtot{\Gamma_\text{tot}}
\def\as{\alpha_s}
\def\az{\alpha_0}
\def\gz{g_0}
\def\w{\vec{w}}
\def\sdag{\Sigma^{\dag}}
\def\s{\Sigma}

% Math operators
\DeclareMathOperator{\br}{BR}
\DeclareMathOperator{\tr}{tr}
\DeclareMathOperator{\Tr}{Tr}
\DeclareMathOperator{\diag}{diag}
\DeclareMathOperator{\Real}{Re}
\DeclareMathOperator{\Imag}{Im}
\DeclareMathOperator{\Pois}{Pois}
\DeclareMathOperator{\cov}{cov}
\DeclareMathOperator{\var}{var}

\newcommand{\Langle}{\big\langle}
\newcommand{\Rangle}{\big\rangle}

\newcommand{\schi}{s_{Z'}}
\newcommand{\cchi}{c_{Z'}}
\newcommand{\tchi}{t_{Z'}}
\newcommand{\sschi}{2 s_{Z'} c_{Z'}}

\newcommand{\psib}{\overline{\psi}}
\newcommand{\Psib}{\overline{\Psi}}
%\newcommand{\dslash}{\not{\hbox{\kern-3pt $\partial$}}}
%\newcommand{\Dslash}{\not{\hbox{\kern-3pt $D$}}}
%\def\one{\leavevmode\hbox{\small1\kern-7.3pt\normalsize1}}
%%\def\one{I}
\newcommand\one{\leavevmode\hbox{\small1\normalsize\kern-.33em1}}
\newcommand{\Mpl}{M_\text{Pl}}
%\def\dslash{\not{\hbox{\kern-4pt $\partial$}}}
%\def\Dslash{\not{\hbox{\kern-4pt $D$}}}
\newcommand{\p}{\partial}
\newcommand{\mat}{\mathcal{M}}
\newcommand{\lag}{\mathcal{L}}
\newcommand{\ord}{\mathcal{O}}
\newcommand{\ope}{\mathcal{O}}
\newcommand{\matx}{|\mathcal{M}|^2}

\newcommand{\qqquad}{\qquad \qquad}
\newcommand{\qqqquad}{\qquad \qquad \qquad}

\newcommand{\qb}{\bar{q}}
\newcommand{\really}{\stackrel{!}{=}}
\newcommand{\msbar}{\overline{\text{MS}}}
\newcommand{\qns}{f_q^\text{NS}}
\newcommand{\lqcd}{\Lambda_\text{QCD}}
\newcommand{\met}{\slashchar{E}_T}
\newcommand{\pmiss}{\slashchar{\vec{p}}_T}

% for SUSY fit projects
\newcommand{\Mzero}{\ensuremath{m_0}}
\newcommand{\MOneHalf}{\ensuremath{m_{1/2}}}
\newcommand{\omegacdm}{\ensuremath{\Omega h^2}}
\newcommand{\Mtop}{\ensuremath{m_t}}
\newcommand{\Mone}{\ensuremath{M_1}}
\newcommand{\Mtwo}{\ensuremath{M_2}}
\newcommand{\Mthree}{\ensuremath{M_3}}
\newcommand{\Deltaamu}{\ensuremath{\text{\Delta a_\mu}}}
\newcommand{\chisq}{{\ensuremath -2\log L}}
\newcommand{\Alambda}{{\ensuremath {A_\lambda}}}
\newcommand{\Akappa}{{\ensuremath {A_\kappa}}}
\newcommand{\tkappa}{{\ensuremath{\tilde \kappa}}}
\newcommand{\abs}[1]{\left |#1\right |}
\newcommand{\unit}[1]{\ensuremath{\, \text{#1}}}

\newcommand{\lsp}{\tilde \chi}
\newcommand{\sq}{\tilde{q}}
\newcommand{\go}{\tilde{g}}
\newcommand{\st}[1]{\tilde{t}_{#1}}
\newcommand{\stb}[1]{\tilde{t}_{#1}^*}
\newcommand{\nz}[1]{\tilde{\chi}_{#1}^0}
\newcommand{\cp}[1]{\tilde{\chi}_{#1}^+}
\newcommand{\cm}[1]{\tilde{\chi}_{#1}^-}
\newcommand{\CP}{CP}

% all the masses 
\providecommand{\mg}{m_{\tilde{g}}}
\providecommand{\mst}[1]{m_{\tilde{t}_{#1}}}
\newcommand{\msn}[1]{m_{\tilde{\nu}_{#1}}}
\newcommand{\mch}[1]{m_{\tilde{\chi}^+_{#1}}}
\newcommand{\mne}[1]{m_{\tilde{\chi}^0_{#1}}}
\newcommand{\msb}[1]{m_{\tilde{b}_{#1}}}
\newcommand{\vsm}{\ensuremath{v_\text{SM}}}

% units of measure
\newcommand{\cmu}{\text{cm}}
\newcommand{\mev}{\text{MeV}}
\newcommand{\gev}{\text{GeV}}
\newcommand{\tev}{\text{TeV}}
\newcommand{\fb}{\text{fb}}
\newcommand{\ab}{\text{ab}}
\newcommand{\pb}{\text{pb}}
\newcommand{\sign}{\text{sign}}
\newcommand{\ifb}{\ensuremath{\text{fb}^{-1}} }
\newcommand{\iab}{\ensuremath{\text{ab}^{-1}} }
\newcommand{\ipb}{\text{pb}^{-1}}

% really great macro by Chris Lester
\def\slashchar#1{\setbox0=\hbox{$#1$}           % set a box for #1
   \dimen0=\wd0                                 % and get its size
   \setbox1=\hbox{/} \dimen1=\wd1               % get size of /
   \ifdim\dimen0>\dimen1                        % #1 is bigger
      \rlap{\hbox to \dimen0{\hfil/\hfil}}      % so center / in box
      #1                                        % and print #1
   \else                                        % / is bigger
      \rlap{\hbox to \dimen1{\hfil$#1$\hfil}}   % so center #1
      /                                         % and print /
   \fi}
\newcommand{\dslash}{\slashchar{\partial}}
\newcommand{\Dslash}{\slashchar{D}}

\newcommand{\eg}{\textsl{e.g.}\;}
\newcommand{\ie}{\textsl{i.e.}\;}
\newcommand{\etal}{\textsl{et al}\;}
%\DeclareMathOperator{\tr}{Tr}

% maximal number of floating environments on each page 
\setlength{\floatsep}{0pt}
\setcounter{topnumber}{1}
\setcounter{bottomnumber}{1}
\setcounter{totalnumber}{1}
\renewcommand{\topfraction}{1.0}
\renewcommand{\bottomfraction}{1.0}
\renewcommand{\textfraction}{0.0}
\renewcommand{\thefootnote}{\fnsymbol{footnote}}

\newcommand{\rig}{\rightarrow}
\newcommand{\lrig}{\longrightarrow}
\renewcommand{\d}{{\text{d}}}
\newcommand{\gl}[1]{(\ref{#1})}
\newcommand{\ta}[2]{ \frac{ {\text{d}} #1 } {{\text{d}} #2}}
\newcommand{\ep}{\varepsilon}
\newcommand{\eps}{\epsilon}
%\renewcommand{\vec}{\bf}
\newcommand{\emt}{$\times 10^{-3}$}
\newcommand{\emfo}{$\times 10^{-4}$}
\newcommand{\emfi}{$\times 10^{-5}$}

\newcommand{\revision}[1]{{\bf{}#1}}

\newcommand{\hzero}{\ensuremath{h^0}}
\newcommand{\Hzero}{\ensuremath{H^0}}
\newcommand{\Azero}{\ensuremath{A^0}}
\newcommand{\PHiggs}{\ensuremath{H}}
\newcommand{\PW}{\ensuremath{W}}
\newcommand{\PZ}{\ensuremath{Z}}

\newcommand{\sw}{\ensuremath{s_w}}
\newcommand{\cw}{\ensuremath{c_w}}
\newcommand{\swd}{\ensuremath{s^2_w}}
\newcommand{\cwd}{\ensuremath{c^2_w}}

%% 2HDM Higgs masses
\newcommand{\mhhd}{\ensuremath{m^2_{\Hzero}}}
\newcommand{\mhh}{\ensuremath{m_{\Hzero}}}
\newcommand{\mlhd}{\ensuremath{m^2_{\hzero}}}
\newcommand{\Mlh}{\ensuremath{m_{\hzero}}}
\newcommand{\mad}{\ensuremath{m^2_{\Azero}}}
% \newcommand{\ma}{\ensuremath{m_{\Azero}}}
\newcommand{\mhpd}{\ensuremath{m^2_{\PHiggs^{\pm}}}}
\newcommand{\mhp}{\ensuremath{m_{\PHiggs^{\pm}}}}

\newcommand{\sa}{\ensuremath{\sin\alpha}}
\newcommand{\ca}{\ensuremath{\cos\alpha}}
\newcommand{\cad}{\ensuremath{\cos^2\alpha}}
\newcommand{\sad}{\ensuremath{\sin^2\alpha}}
\newcommand{\sbd}{\ensuremath{\sin^2\beta}}
\newcommand{\cbd}{\ensuremath{\cos^2\beta}}
\newcommand{\cb}{\ensuremath{\cos\beta}}
\renewcommand{\sb}{\ensuremath{\sin\beta}}
\newcommand{\tanbd}{\ensuremath{\tan^2\beta}}
\newcommand{\cotbd}{\ensuremath{\cot^2\beta}}
\newcommand{\tanb}{\ensuremath{\tan\beta}}
\newcommand{\tb}{\ensuremath{\tan\beta}}
\newcommand{\cotb}{\ensuremath{\cot\beta}}

\newcommand{\Sherpa}{S\protect\scalebox{0.8}{HERPA}\xspace}

\newcommand{\brinv}{\ensuremath{BR_{\text{inv}}}\xspace}
\newcommand{\vegas}{\textsc{Vegas}\xspace}
\newcommand{\madgraph}{\textsc{Madgraph}5\xspace}
\newcommand{\pythia}{\textsc{Pythia}\xspace}
\newcommand{\fastjet}{\textsc{FastJet}\xspace}
\newcommand{\delphes}{\textsc{Delphes}\xspace}
\newcommand{\sherpa}{\textsc{Sherpa}\xspace}
\newcommand{\sklearn}{\textsc{scikit-learn}\xspace}
\newcommand{\keras}{\textsc{Keras}\xspace}
\newcommand{\theano}{\textsc{Theano}\xspace}
\newcommand{\adam}{\textsc{Adam}\xspace}
\newcommand{\etmiss}{\ensuremath{E_T^{\text{miss}}}\xspace}
\newcommand{\lumi}{\ensuremath{\mathcal{L}}\xspace}
\newcommand{\sqrts}{\ensuremath{\sqrt{s}}\xspace}

% Define commenting commands
\newcommand{\Felix}[1]{\textcolor{magenta}{FK:#1}}
\newcommand{\FK}[1]{\textcolor{Magenta}{{[ FK: #1]}}}
\newcommand{\PR}[1]{\textcolor{Green}{{[ PR: #1]}}}
\newcommand{\PF}[1]{\textcolor{RoyalBlue}{{[ PF: #1]}}}
